Semantic Guidance and Feedback for the Construction of Specifications and Implementations

The problem of writing a specification which accurately reflects the intent of the developer has long been recognized as fundamental. We propose a method and a supporting tool to write and check a specification and an implementation using a set of use cases, \ie input-output pairs that the developer supplies. These are instances of both good (correct) and bad (incorrect) behavior. We assume that the use cases are accurate, as it is easier to generate use cases than to write an accurate specification. We incrementally construct a specification (precondition and postcondition) based on semantic feedback generated from these use cases. We check the accuracy of the constructed specification using two proposed algorithms. The first algorithm checks the accuracy of the specification against an automatically generated specification from a supplied finite domain of use cases. The second checks the accuracy of the specification via reducing its domain to a finite yet equally satisfiable domain if possible. When the specification is mature, we start to also construct a program that satisfies the specification. However, our method makes provision for the continued modification of the specification, if needed. We illustrate our method with two examples; linear search and text justify.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{relsize}
\usepackage{fancyvrb}
\usepackage{ifthen}
\usepackage{multirow}

\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{latexsym}

\RequirePackage{xspace}
\RequirePackage{url}

\usepackage[pdftex]{graphicx}

\RequirePackage{color}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations
\newcommand{\tf}{\ensuremath{\{\true, \false\}}}




%%%%%%%%%%%%%%%%%%%%%%%% Lists
\newcommand{\be}{\begin{itemize}}
\newcommand{\ee}{\end{itemize}}
\newcommand{\bdn}{\begin{description}}
\newcommand{\edn}{\end{description}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\renewcommand{\i}{\item}

\newenvironment{closeitemize}{\begin{list}%
{$\bullet$}%
{\setlength{\itemsep}{-0.2\baselineskip}%
\setlength{\topsep}{0.2\baselineskip}}}%
{\end{list}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MISC

\newcommand{\remove}[1]{}

\newcommand{\case}[2]{\vspace{1.5ex} \noindent \textit{Case} #1: \emph{#2}.}
\newcommand{\scase}[2]{\vspace{1.5ex} \noindent \textit{Subcase} #1: #2.}
\newcommand{\sscase}[2]{\vspace{1.0ex} \noindent \textit{Subsubcase} #1: #2.}

%\newcommand{\defn}[1]{\textit{#1}}
\newcommand{\defi}[1]{\textit{#1}:}



%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES AND THEOREMS


\newtheorem{definition}{Definition}[]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\renewcommand{\thefootnote}{\arabic{footnote}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text
\newcommand{\smpage}{\noindent \parbox{\textwidth}}
\newcommand{\samep}{\parbox{\textwidth}}   % put onto the same page


\newcommand{\mathid}[1]{\ensuremath{\mathit{#1}}\xspace}

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\ul}{\underline}
\newcommand{\bs}{\bigskip}
%\newcommand{\ms}{\medskip}
%\renewcommand{\ss}{\smallskip}

\newcommand{\bfg}{\begin{figure}}
\newcommand{\efg}{\end{figure}}

\renewcommand{\ss}{\smallskip}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}


\newcommand{\intr}{\empi}
\newcommand{\intrdef}{\emph}

\newcommand{\emp}[1]{\textbf{#1}}
\newcommand{\empp}[1]{\emph{#1}}
\newcommand{\empb}[1]{\textbf{#1}}
\newcommand{\empi}[1]{\textit{#1}}
\newcommand{\empbi}[1]{\textbf{\textit{#1}}}

\newcommand{\ind}{\hspace*{3.0em}}

%%%%%From Nancy's book directory:  This spaces the symbols within a
%%%%%word nicely, in math mode.
\newcommand{\ms}[1]{%
        \relax\ifmmode
                \mathord{\mathcode`\-="702D\it #1\mathcode`\-="2200}%
        \else
                $\mathord{\mathcode`\-="702D\it #1\mathcode`\-="2200}$%
        \fi
}


\newcommand{\cmnt}{\`}


%%%%%%%%%%%%%%%%%%%%%%% GENERAL MATH SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Adj}{\mathop{\rm Adj}\nolimits}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\card}[1]{\left| #1\right|}
\newcommand{\ar}{\rightarrow}
%\newcommand{\ar}{\longrightarrow}
\newcommand{\al}{\alpha}
\renewcommand{\b}[1]{\overline{#1}}
\newcommand{\cat}{\mathbin{\frown}}
\newcommand{\choice}{\mbox{$[\hspace*{-1.0pt}]$}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\renewcommand{\d}{\, . \,}      % separator in quantified formulae
\newcommand{\df}{\triangleq}
%\newcommand{\df}{\mbox{$\:\stackrel{\rm df}{=\!\!=}\:$}}
\newcommand{\dn}{\mbox{$\hspace{-0.1em}\downarrow\hspace{-0.1em}$}}
\newcommand{\Ex}{\mathop{\rm Ex}}
\newcommand{\es}{``"}   %empty string
\newcommand{\expect}[1]{{\rm E}\left[ #1 \right]}
\newcommand{\expectsq}[1]{{\rm E}^2\left[ #1 \right]}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\renewcommand{\ge}{\geqslant}
\newcommand{\given}{\mid}
\newcommand{\halfind}{\hspace*{1.5em}}
\newcommand{\ifof}{\Longleftrightarrow} % logical equivalence
\newcommand{\img}{\mathrm{Image}}
\newcommand{\ints}{\cap}
\renewcommand{\l}{\ell}
\newcommand{\la}[1]{\mbox{$\, \stackrel{#1}{\rightarrow} \,$}}
\renewcommand{\le}{\leqslant}
\newcommand{\lra}{\mbox{$\longrightarrow$}}
%\newcommand{\mod}{\ \mathrm{mod}\ }
\newcommand{\oneton}{\{1,\,\ldots, n\}}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\prob}[1]{\Pr\left\{ #1 \right\}}
\newcommand{\pind}{\hspace*{3.0em}}
\newcommand{\pj}{\!\upharpoonright\!}
\newcommand{\proj}{\pj}
\newcommand{\preimg}{\mathrm{PreImage}}
\newcommand{\pl}{\!\parallel\!}
\newcommand{\s}{\mbox{$\hspace{-1pt}-\hspace{-2pt}$}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
%\newcommand{\set}[1]{\{#1\}}
\newcommand{\seq}{\approx}
\newcommand{\spc}{\mbox{\vspace{-0.25in}}}
\newcommand{\st}[2]{\mbox{$\stackrel{#1}{#2}$}} % abbreviated stackrel
%\newcommand{\st}{\ | \ }
\newcommand{\sub}{\subseteq}
\newcommand{\twodots}{\mathinner{\ldotp\ldotp}}
\newcommand{\tiff}{\textup{\ iff\ }}
\newcommand{\tl}[1]{\mbox{$\tilde{#1}$}}% abbreviated tilde
\newcommand{\tpl}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\un}{\cup}
\newcommand{\union}{\bigcup}
\newcommand{\up}{\mbox{$\hspace{-0.1em}\uparrow\hspace{-0.1em}$}}
\newcommand{\Var}{\mathop{\rm Var}\nolimits}
\newcommand{\variance}[1]{{\rm Var}\left[ #1 \right]}
\newcommand{\w}{\omega}


%%%%%%%%%%%%%%%%%%% Ints, Reals, etc %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\reals}{{\mathbb R}}
\newcommand{\integers}{{\mathbb Z}}
\newcommand{\naturals}{{\mathbb N}}
\newcommand{\nat}{\naturals}
\newcommand{\nats}{\naturals}
\newcommand{\rationals}{{\mathbb Q}}
\newcommand{\complex}{{\mathbb C}}
\newcommand{\complexes}{{\mathbb C}}



%%%%%%%%%%%%%%%%%%%%%%%%% MATH MACROS AND ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\se}[3]{\ensuremath{#1[#2 .. #3]}}
\newcommand{\se}[3]{\ensuremath{#1[#2 \! : \! #3]}}
%\newcommand{\se}[3]{\ensuremath{#1[#2,\ldots,#3]}}


\newcommand{\ang}[1]{\ifmmode{\left\langle #1 \right\rangle}
   \else{$\left\langle${#1}$\right\rangle$}\fi}
        % the \if allows use outside mathmode,
        % but will swallow following space there!

\newcommand{\struct}[2]{\raisebox{-0.1in}{$\stackrel { \displaystyle
#1} {\scriptstyle #2}\,$}}

\newcommand{\pbx}[2]{\stackrel{\fbox{\begin{Beqnarray*} #1\\.\\.\\.\\#2 \end{Beqnarray*}}}{}}      % proof box



%%%%%%%%%%%%%%%%%%%%%%% Hoare Logic Symbols
\newcommand{\lng}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\htp}[3]{\ensuremath{\{#1\}\,#2\,\{#3\}}}
\newcommand{\htptc}[3]{\ensuremath{\langle#1\rangle\,#2\,\langle#3\rangle}}
\newcommand{\var}{\ensuremath{\varphi}}

\newcommand{\as}[1]{\ensuremath{\{#1\}}}               % partial correctness asserion
\newcommand{\ts}[1]{\ensuremath{\langle #1 \rangle}}   % termination correctness asserion

\newcommand{\ch}{\mbox{[\hspace{-0.15ex}]}}

\newcommand{\pa}[1]{\{\ensuremath{#1}\}}
%\newcommand{\ta}[1]{$<$#1$>$}
\newcommand{\ta}[1]{$\langle$\ensuremath{#1}$\rangle$}

\newcommand{\pre}[1]{\textsf{Precondition: #1}}
\newcommand{\post}[1]{\textsf{Postcondition: #1}}

\newcommand{\satt}{\equiv}
\newcommand{\sat}{\models}

\newcommand{\yld}{\vdash}
\newcommand{\yldd}{\equiv}
%\newcommand{\yldd}{\dashv \vdash}






\newcommand{\pc}[1]{{#1}}    %% font for pseudocode
%\newcommand{\pc}[1]{\codetext{#1}}    %% font for pseudocode

%%%%%%%%%%%%%% MACROS FOR NUMBERED LINES IN CODE TABBING ENVIRONMENT %%%%%%%%%%%%%%%%

\newcounter{lctr}

\newcommand{\li}{\addtocounter{lctr}{1}\arabic{lctr}.}
\newcommand{\lio}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\ensuremath{#1}\\}
\newcommand{\lit}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\ensuremath{#1}\\}
\newcommand{\lih}[1]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\>\ensuremath{#1}\\}

%%%% 2'nd argument is for a commment
\newcommand{\lioc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\ensuremath{#1}\`{#2}\\}
\newcommand{\litc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\ensuremath{#1}\`{#2}\\}
\newcommand{\lihc}[2]{\addtocounter{lctr}{1}\arabic{lctr}.\>\>\>\ensuremath{#1}\`{#2}\\}




%%%%%%%%%%%%%%%%%%%%%%%%%%% PSEUDOCODE SECTION

\newcommand{\gt}{\ensuremath{:=}}   % assignment
%\newcommand{\gt}{\ensuremath{\leftarrow}}   % assignment
\newcommand{\swap}{\ensuremath{\leftrightarrow}}   % swap two vars

\newcommand{\pseudocode}[1]{\ensuremath{\mathbf{#1}\ }}
\newcommand{\pseudocodensp}[1]{\ensuremath{\mathbf{#1}}}
%\newcommand{\pseudocode}[1]{\mbox{${\bf #1}$}\xspace}

\newcommand{\IFC}[1]{\pseudocode{if}\ (\ensuremath{#1})}
\newcommand{\WHILEC}[1]{\pseudocode{while}\ (\ensuremath{#1})}
\newcommand{\RETURNE}[1]{\pseudocodensp{return}(\ensuremath{#1})}

\newcommand{\IF}{\pseudocode{if}}
\newcommand{\FI}{\pseudocode{fi}}
\newcommand{\THEN}{\pseudocode{then}}
\newcommand{\ELSE}{\pseudocode{else}}
\newcommand{\ELSF}{\pseudocode{else\ if}}
\newcommand{\ENDIF}{\pseudocode{endif}}

\newcommand{\WHILE}{\pseudocode{while}}
\newcommand{\ENDWHILE}{\pseudocode{endwhile}}
\newcommand{\FOR}{\pseudocode{for}}
\newcommand{\FORALL}{\pseudocode{forall}}
\newcommand{\ENDFOR}{\pseudocode{endfor}}
\newcommand{\DO}{\pseudocode{do}}
\newcommand{\OD}{\pseudocode{od}}

\newcommand{\BEGIN}{\pseudocode{begin}}
\newcommand{\END}{\pseudocode{end}}
\newcommand{\PROC}{\pseudocode{procedure}}
\newcommand{\CALL}{\pseudocode{call}}
\newcommand{\VAL}{\pseudocode{value}}
\newcommand{\VALRES}{\pseudocode{value\!-\!result}}
\newcommand{\RES}{\pseudocode{result}}
\newcommand{\RETURN}{\pseudocode{return}}
\newcommand{\DOWNTO}{\pseudocode{downto}}
\newcommand{\TO}{\pseudocode{to}}

\newcommand{\function}{\pseudocode{function}}
\newcommand{\operation}{\pseudocode{operation}}

\newcommand{\newo}{\pseudocode{new}}
\renewcommand{\int}{\pseudocode{int}}







%%%%%%%%%%%%%%%%%%%%%%%%%%%% Boolean Constants

\newcommand{\T}{\mbox{\rm T}}
\newcommand{\F}{\mbox{\rm F}}
\newcommand{\Fa}{\mbox{\rm F}}

\newcommand{\true}{\ensuremath{\mathit{true}}}
%\newcommand{\true}{\mbox{\textsc{true}}\xspace}
\newcommand{\false}{\ensuremath{\mathit{false}}}
%\newcommand{\false}{\mbox{\textsc{false}}\xspace}

%\newcommand{\TT}{\top}
%\newcommand{\FF}{\bot}

\newcommand{\TT}{\mathit{true}}
\newcommand{\FF}{\mathit{false}}

\newcommand{\ANDW}{\mbox{\bf and \xspace}}
%\newcommand{\OR}{{\bf or} }
%\newcommand{\NOT}{{\bf not} }




%%%%%%%%%%%%%%%%%%%%%%%%% Boolean Connectives

\renewcommand{\iff}{\equiv}
%\renewcommand{\iff}{\Leftrightarrow}
\newcommand{\imp}{\Rightarrow}
\newcommand{\ev}{\equiv}
%\newcommand{\implies}{\Rightarrow}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% QUANTIFIERS

\newcommand{\qt}[3]{#1\,#2\,#3}
\newcommand{\qtr}[4]{(#1\,#2 : #3 : #4)}

\newcommand{\Q}{\mbox{${\bf Q}$}\xspace}
\newcommand{\q}{\mbox{${\bf q}$}\xspace}

%% quantifiers
\newcommand{\AND}{\bigwedge}
\newcommand{\INTER}{\bigcap}
\newcommand{\OR}{\bigvee}
\newcommand{\UN}{\bigcup}
\newcommand{\SUM}{\Sigma}
%\newcommand{\INT}{\bigcap}

%% Logical Quantifiers
\newcommand{\fa}{\ensuremath{\forall\,}}
%\newcommand{\fa}{\mbox{${\mathbf{\forall}}$}\xspace}
\newcommand{\ex}{\ensuremath{\exists\,}}
%\newcommand{\ex}{\mbox{${\mathbf{\exists}}$}\xspace}

\newcommand{\LQ}{\mbox{${\bf LQ}$}\xspace}


%% Arithmetic Quantifiers
%\renewcommand{\S}{\Sigma\,}
%\renewcommand{\S}{\mbox{${\mathbf{\Sigma}}$}\xspace}
\renewcommand{\P}{\Pi\,}
\newcommand{\N}{\ensuremath{\mathrm{N}\,}}
\newcommand{\AQ}{\ensuremath{\mathrm{AQ}\,}}
\newcommand{\MAX}{\ensuremath{\mathrm{MAX}\,}}
\newcommand{\MIN}{\ensuremath{\mathrm{MIN}\,}}


%% Predicate Logic Symbols
\newcommand{\FS}{\mathcal{F}}
\newcommand{\PS}{\mathcal{P}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Sp}{\mathcal{S}}             % specification
\newcommand{\E}{\mathcal{E}}
\newcommand{\B}{\mathcal{B}}


%%%%%%%%%%%%%%%%%%%%%% Temporal Logic

\newcommand{\G}{\Box}
\newcommand{\Gl}{\Box}
%\newcommand{\F}{\diamond}
\newcommand{\Fl}{\diamond}





%%%%%%%%%%%%%%%%% EQUATION ENVIRONMENTS
\newcommand{\beqn}{\begin{centeqn}}
\newcommand{\eeqn}{\end{centeqn}}
\newcommand{\beqnnbsp}{\begin{centeqn-nbsp}}
\newcommand{\eeqnnbsp}{\end{centeqn-nbsp}}
\newcommand{\bleqn}[1]{\begin{centlabeqn}{#1}}
\newcommand{\eleqn}{\end{centlabeqn}}
\newcommand{\bleqnnbsp}[1]{\begin{centlabeqn-nbsp}{#1}}
\newcommand{\eleqnnbsp}{\end{centlabeqn-nbsp}}

\newenvironment{centeqn}	% centered equation environment
   {{\ss\\ \hspace*{\fill}}}
   {\hspace*{\fill}\ss\\}

\newsavebox{\EqnLabel}
\newenvironment{centlabeqn}[1]	% centered labeled equation environment
   {\sbox{\EqnLabel}{#1}
    {\bs\\ \hspace*{\fill}}
   }
   {\hfill{\makebox[0in][r]{\usebox{\EqnLabel}}}\bs\\}

\newenvironment{centeqn-nbsp} % centered equation - no vertical space at the bottom
   {{\medskip\\ \hspace*{\fill}}}
   {\hspace*{\fill}}




%%%%%%%%%%%%%%%% SpecCheck Specific macros

\newcommand{\cd}[1]{{\small\texttt{#1}}}
\newcommand{\cci}[1]{{\small\texttt{#1}}}
%\newcommand{\chci}[1]{`\cci{#1}'}
\newcommand{\chci}[1]{\cci{#1}}

\newcommand{\good}{\cci{good}\xspace}
\newcommand{\bad}{\cci{bad}\xspace}
\newcommand{\tgood}{\tiny\texttt{good}\xspace}
\newcommand{\tbad}{\tiny\texttt{bad}\xspace}
\newcommand{\dc}{\cci{dontCare}\xspace}
\newcommand{\tdc}{\tiny\texttt{dontCare}\xspace}

\newcommand{\ord}{\sqsubseteq}
\newcommand{\ordne}{\sqsubset}

\newcommand{\white}{\ensuremath{\mathit{white}}\xspace}
\newcommand{\black}{\ensuremath{\mathit{black}}\xspace}

\newcommand{\ls}{\cd{ls}}
\newcommand{\af}{f}



